Rapidly Adaptable Legged Robots via Evolutionary Meta-Learning

Learning adaptable policies is crucial for robots to operate autonomously in our complex and quickly changing world. In this work, we present a new meta-learning method that allows robots to quickly adapt to changes in dynamics. In contrast to gradient-based meta-learning algorithms that rely on second-order gradient estimation, we introduce a more noise-tolerant Batch Hill-Climbing adaptation operator and combine it with meta-learning based on evolutionary strategies. Our method significantly improves adaptation to changes in dynamics in high noise settings, which are common in robotics applications. We validate our approach on a quadruped robot that learns to walk while subject to changes in dynamics. We observe that our method significantly outperforms prior gradient-based approaches, enabling the robot to adapt its policy to changes based on less than 3 minutes of real data.

==> ignorethis_storage.tex <==
\ignorethis{We first state some of the sources of noise, which include random initializations, changing of dynamics over the course of real-world training (e.g. due to motor overheating and battery level dropping), potential catastrophic hardware failure (where the reward is extremely low), and observation noise due to inaccurate sensors. Such examples suggest the noise is no longer independent throughout real-world adaptation. Due to these types of failure cases, }

\ignorethis{
To operate autonomously in the fast changing world, robots need to adapt effectively to changes in the environment. Deep reinforcement learning (RL) has led to voluminous literature on training RL policies maximizing rewards for specific well-defined tasks. In comparison, much less effort was devoted to learning policies that can easily adapt to tasks that are potentially not even defined in training. Model-Agnostic Meta-Learning (or simply MAML/meta-RL) aims to learn such policies \cite{PG-MAML}. However, most works focus on differentiating tasks by changing the reward function, where the adaptation signal is clear and the optimal policy for each task is necessarily different. A primary motivation for this work is the following question:

\begin{center}
\textit{How do we ensure effective adaptation in adversarial high-noise environments when the dynamics, not the rewards, are being altered? }
\end{center}
}
\ignorethis{Physical simulation for real world transfer (Sim2Real) has recently been an important paradigm for robot learning, especially through the use of domain randomization \citep{}. However, it requires implicit assumptions, which we enumerate:

\textbf{The tasks encountered in simulation have relatively little domain shift to real world tasks.} This assumption can be quite strict and resource intensive, requiring simulation of a very large range of possible scenarios in order to truly interpolate a real world scenario. In real life, sudden domain shifts occur often without knowing in advance, sometimes different from the simulated training distribution.

\textbf{There exists a single policy which can solve all tasks from both simulation/training and real-world/testing.} This condition is straightforward for feed-forward convolutional networks, where extra tasks involving differing colors and backgrounds (i.e. data augmentation) allows the policy to be invariant to irrelevant objects. However, changes between training and testing which involve changes in dynamics, such as differing gravity and friction potentially may not be solved by a single feed-forward policy, but may require an RNN instead to satisfy this condition. Such RNN policies can be quite large with thousands of parameters requiring an on-board GPU, uninterpretable, and data-intensive, which may be impractical for certain robotics use cases, such as a Minitaur. 

These two assumptions suggest that a learned adaptation behavior with a compact policy can potentially be more data-efficient and solve a wider range of tasks not encountered in simulation. An promising method to achieve this goal is to pretrain the policy in simulation by using gradient-based adaptation methods, such as MAML \citep{} which has seen significant results in the areas of supervised learning and deep reinforcement learning. The MAML algorithm seeks to find a "meta-policy" for it is easy to perform a gradient-update using few extra data from a given task (i.e. trajectories) which results in a final adapted policy optimal for said task.

However, one subtle but interesting challenge we discuss in this work, is to not allow the meta-policy to solve all tasks immediately in simulation, as this would imply the policy has not learned how to adapt (as there is no need to). We instead desire the meta-policy to be reasonably decent, but not exceedingly robust such that it is unable to adapt to domain shifts in the real world. In this work, we find that directly applying the vanilla policy-gradient variant of MAML for RL "PG-MAML" is not sufficient, as PG-MAML encounters this problem very often. Instead, we use a more recently developed "ES-MAML" \citep{} based on ARS and ES \citep{} which eventually allows for both quantitative and qualitative evidence of adaptation.

The main contributions of this work are: (1) demonstrating the need for adaptation when there are domain shifts in the dynamics for a legged robot, (2) analyzing the effects of strong environment stochasticity on adaptation algorithms, and (3) showing the effectiveness of MAML on real world tasks.}

\ignorethis{Although PG-MAML has been demonstrated in a number of simulation benchmarks, its application to real-world domain adaptation has been limited. We hypothesize this as a result of two reasons:

First, to effectively perform adaptation, PG-MAML needs a sufficiently deep policy representation \cite{maml-and-universality}. Since in our dynamics setting, we are looking at changes in transition dynamics and not the reward function, an improved representation power in the policy will likely lead to domain randomization. Moreover, the noise in real world environments can significantly degrade the performance of vanilla MAML-based approaches. These weaknesses suggest that a stable compact policy is needed, one whose optimization process can also be easily modified to adapt against noise.}

\ignorethis{
We used the following hyperparameters in our training setup in Table \ref{table:hyperparameters}.
\begin{table}[h]
    \centering
    \scalebox{1}{
    \begin{tabular}{|c|c|}
    \hline
       \textbf{Parameter}  & \textbf{Value} \\
       \hline\hline
        (Total Workers, Perturbations, Test Workers) & (450, 300, 100) \\\hline
        Adaptation Step Size $\alpha$ & 0.05 \\\hline
        Outer-Loop Step Size $\beta$ & 0.01 \\\hline
        Adaptation Precision Parameter & 0.1 \\\hline
        Outer-Loop Precision Parameter & 0.1 \\\hline
    \end{tabular}
    }
    \caption{\label{table:hyperparameters}Hyperparameters used.}
\end{table}
For training stability purposes, ES-MAML uses state normalization and reward normalization, both features common to \cite{ARS, ES-MAML}. 
}


\ignorethis{

Here the loss function for meta-training is given as an average loss over tasks from $\mathcal{T}$ after the aforementioned gradient-step adaptations. Training as well as adaptation is conducted using policy gradient methods. We will refer to the entire algorithm as PG-MAML.  Since PG-MAML was published, several improvements of the algorithm were proposed: via stochastic gradient adaptation \cite{finn}, by omitting
second derivatives resulting in a simplified and cheaper implementation (First-Order MAML or FOMAML), by simplifying PG-MAML with multiple gradient steps on the randomly sampled task followed by policy parameters' updates performed repeatedly ($\mathrm{Reptile}$, \cite{nichol}) and more.

Surprisingly, all these methods were so far tested to be successful only on relatively simple simulated environments and to the best of our knowledge no results on the effectiveness of those algorithms on hardware were reported. 
The reason is that, as we demonstrate in Section \ref{sec:experiments}, gradient-based methods that can operate only with differentiable adaptation operators are simply inadequate to work in real environments characterized by high adversarial noise, where wrongly chosen policy configurations can lead to potentially catastrophic failures.


Meta RL papers:
\begin{itemize}
    \item \cite{PG-MAML}: original PG-MAML paper
    \item A series of PG-MAML improvements that analyzes the issue of PG-MAML on RL.
    \item \cite{ES-MAML}: ES-MAML paper.
\end{itemize}

Domain Adaptation in (real) robotics
\begin{itemize}
    \item \cite{sim-to-real, peng2018sim}: Domain Randomization for transfer / robust.
    \item \cite{meta-strategy-optimization}: Wenhao's paper, requires domain knowledge
    \item \cite{arndt2019meta}: Sim-to-real demonstrated on arm, where the task is signficantly easier.
\end{itemize}
}


\ignorethis{
We first discuss the original formulation of MAML \cite{PG-MAML}. Let $\mathcal{T}$ be a set of reinforcement learning tasks with common state and action spaces $\mathcal{S}, \mathcal{A}$, and $\mathcal{P}(\mathcal{T})$ a distribution over $\mathcal{T}$. In the standard MAML setting, each task $T_{i} \in \mathcal{T}$ has an associated Markov Decision Process (MDP) with transition distribution $q_{i}(s_{t+1}|s_{t},a_{t})$, an episode length $H$, and a reward function $\mathcal{R}_{i}$ which maps a trajectory $\tau = (s_{0},a_{1},...,a_{H-1},s_{H})$ to the total reward $\mathcal{R}(\tau)$. A \emph{stochastic policy} is a function $\pi : \mathcal{S} \rightarrow \mathcal{P}(\mathcal{A})$ which maps states to probability distributions over the action space. A \emph{deterministic policy} is a function $\pi: \mathcal{S} \rightarrow \mathcal{A}$. Policies are typically encoded by a neural network with parameters $\theta$, and we often refer to the policy $\pi_\theta$ simply by $\theta$.

The MAML problem is to find the so-called \emph{MAML point} (called also a \textit{meta-policy}), which is a policy $\theta^{*}$ that can be `adapted' quickly to solve an unknown task $T \in \mathcal{T}$ by taking a (few)\footnote{We adopt the common convention of defining the adaptation operator with a single gradient step to simplify notation, but it can readily be extended to taking multiple steps.\nopagebreak} policy gradient steps with respect to $T$. The optimization problem to be solved in training (in its one-shot version) is thus of the form:

where: $\theta^{\prime} = U(\theta, T) = \theta + \alpha \nabla_{\theta}\mathbb{E}_{\tau \sim \mathcal{P}_{T}(\tau | \theta)} [R(\tau)]$ is called the \emph{adapted policy} for a step size $\alpha > 0$ and $\mathcal{P}_{T}(\cdot|\eta)$ is a distribution over trajectories given task $T \in \mathcal{T}$ and conditioned on the policy parameterized by $\eta$.
}
\ignorethis{
These include: 
\textcolor{red}{This is probably redundant}
\begin{center}
\begin{tabular}{ |m{2cm}|m{2cm}|m{2cm}| } 
\hline
Adaptation Name & Meta & Adapted \\
\hline\hline
Overfitting to Horizon & Stops at 500 steps (3s) &  Continues for full horizon length \\
\hline
Correcting Falling Down &  Falls when dynamics are too unstable & Continues for full horizon length \\
\hline
Correcting Turning (Left) & Strongly Curves to the right & Straightens Trajectory \\
\hline
Correcting Turning (Right) & Strongly curves to the left & Straightens Trajectory \\
\hline
\end{tabular}
\end{center}
}


\ignorethis{However, this analysis can be extended to even the adversarial case, under the following assumptions: our parameter dimension is $d$ and we apply our batch method for $T$ iterations, and at every iteration, at most $W$ $(W<P)$ perturbations possess unbounded negative error $\varepsilon$ and the remaining $P-W$ we have $|\varepsilon| \le \Lambda$. We can show that with a high enough $P \ge W + poly(s,d,T)$ there is a high probability $1 - poly(T, \frac{1}{s})$ that we achieve no-regret convergence, i.e. $\frac{1}{T}\sum_{t=0}^{T-1}(f(\theta^{OPT})-f(\theta_t)) \leq \bigO(\frac{1}{\sqrt{T}})$ where the constants in $\bigO(\frac{1}{\sqrt{T}})$ rely on properties of the concavity of $f$. This comes from the fact that there is a high probability at least one of the sampled perturbations $\mathbf{g}_{t}^{i}$ has at most a constant $\phi$ angular distance $\text{angle}(\mathbf{g}_{t}^{i}, \nabla f(\theta_{t})) \le \phi$ to the true gradient $\nabla f(\theta_{t})$, with a high probability of being chosen by the $\argmax$. This implies with a reasonable scaling $\sigma = \alpha$, the picked direction $\theta_{t+1} - \theta_{t} = \sigma\mathbf{g}_{t}^{j^{*}}$ is also close to $\eta_{t} \nabla f(\theta_{t})$ in $\ell_{2}$ norm for some decreasing learning rate $\eta_{t}$, and thus we may use a standard gradient-ascent proof to show convergence. We show this formally in the $\mathrm{arxiv}$ version of this paper in the Appendix. While this proof requires particular conditions on $P$, in practice our method still remains effective if we use a reasonable $P$.}

\ignorethis{
\textcolor{red}{Emphasize what is novel and hasn't been done before here}
\textcolor{red}{How is our work different from https://arxiv.org/pdf/1909.12995.pdf? YXYANG: "One point we can make about ES-MAML vs the Meta Strategy Optimization paper is that the later requires a lot of domain knowledge
Like the ground-truth dynamics params is part of the policy network's input
While ES-MAML learns (and generalizes to unseen dynamics) autonomously"}

We discuss two significant differences in our work from previous works on MAML. 

(1) The performance of MAML-based algorithms are traditionally benchmarked on toy environments and the Mujoco set of benchmarks, where the difference between tasks are entirely due to changes in the reward functions. However, there is a dearth of work on task diversity caused by changes in \textit{dynamics}, which can be more common in real-world scenarios. Generally, it is more clear that in task with different reward functions, the optimal policies for each task are necessarily different (e.g. one cannot joint-train a feed-forward policy on the Forward-Backward tasks from \cite{}). However, this becomes unclear in the varying dynamics case, where there may still exist fixed policies which achieve high performance across multiple tasks when using vanilla joint training. Thus the question rises: what is the purpose of meta-learning then, if one can already joint train on a set of tasks? We answer this by showing that performance across \textit{test tasks} varies significantly as we shift domains, decreasing especially when there is domain shift between training and testing. This case necessitates the need for fast adaptation, whose algorithms we analyze in this work.

(2) The classic Mujoco meta-learning benchmarks also use \textit{deterministic} dynamics. In contrast, both our simulations and real world environments possess significant stochasticity and noise, which affects meta-learning performance dramatically.
}

\ignorethis{
\textcolor{red}{Furthermore, the steps in the HillClimbing operator are \textit{Gaussian}, which enjoys dimensionality reduction properties - if $f(\theta) = g(P_{A} \theta)$ where $P_{A}$ is a projection matrix, then the convergence rate of $f$ is dependent on the low dimensionality of $g$, based on the fact that an affine transformation of a Gaussian is still a Gaussian.}}


\ignorethis{\textcolor{red}{In particular, if $f(\theta) = g(P_{A} \theta) + h(\theta)$ where $P_{A}$ is a projection matrix, the convergence rate of the Batch HillClimbing algorithm is within the convergence rate of $g(\cdot)$. Furthermore in the noiseless case, the "average" method wastes queries, while the Batch algorithm does not}}

\ignorethis{
We formalize the HillClimbing operator below, with general update rules: \textcolor{red}{TODO}
\begin{minipage}{0.47\textwidth}
\begin{algorithm}[H]
\SetAlgoLined
\KwData{Meta-Policy $\theta_{meta}$, adaptation step size $\alpha$, Task $T_{i}$, Parallel Evaluation Parameter $P$}

$v_{max} = f^{T_{i}}(\theta_{meta})$, $\theta_{max} = \theta_{meta}$

\For{$q = 0,1,\ldots Q$}{
    Sample $P$ i.i.d. perturbations $\mathbf{g}_{1},\ldots,\mathbf{g}_{P} \sim \mathcal{N}(0,\mathbf{I})$\;
    
    \ForEach{$\mathbf{g}_{i}$}
    {
        $v_i \gets f^{T_{i}}(\theta_{q} + \alpha g_{i})$
        
        \If{$v_{i} > v_{max}$}
        {
        $v_{max} = v_{i}$
        
        $\theta_{max} = \theta_{q} + \alpha g_{i}$  
        }
    }
    $\theta_{q+1} \gets \theta_{max} $
 }
\caption{General HillClimb Adaptation Operator $U_{batch}(\cdot, T)$ }
\label{algo:hillclimb_adaptation}
\end{algorithm}
\end{minipage}
}


\ignorethis{
\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/qualitative_horizon.pdf}
        \caption{\label{fig:qualitative_horizon}Walking Height}
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/qualitative_height.pdf}
        \caption{\label{fig:qualitative_height}Walking Height}
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/qualitative_turn_left.pdf}
        \caption{\label{fig:qualitative_turn_left}x-y trajectory}
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/qualitative_turn_right.pdf}
        \caption{\label{fig:qualitative_turn_right}x-y trajectory}
    \end{subfigure}
    \caption{Examples of ES-MAML adaptation in the Minitaur simulation environment. Fig.~\ref{fig:qualitative_horizon},\ref{fig:qualitative_height}: HC corrects the robot from falling, leading to longer and more stable walking behavior. Fig.~\ref{fig:qualitative_turn_left},\ref{fig:qualitative_turn_right}: HC corrects the robot from turning left or right.}
    \label{fig:qualitative_adaptation}
\end{figure}
}

\ignorethis{
\subsection{Effectiveness of Compact Policies}
We conjecture the effectiveness of adaptation as partially a result of the compact policy classes used. To validate this, we further re-train the policy with additional hidden layer networks. We found that adding hidden layers always produces a knee-bending behavior, as shown by the significantly higher pitch-angle in Fig.~\ref{fig:pitch_angle}. While the knee-bending behavior does achieve a good reward in most cases, it does not transfer to real robot due to the difference in contact dynamics. 

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{images/pitch_angle.png}
    \caption{Robot pitch angle for policy trained with one hidden layer. The robot bends its front legs and crawled forward, which results in significantly larger pitch angles.}
    \label{fig:pitch_angle}
\end{figure}

The phenomenon of linear policies working well with ES-based methods has been observed numerous times in previous works. For example, linear policies for ES outperform policy gradients in Mujoco \cite{ARS}, and have been used to show reverse trends between performance and architecture size for meta-learning when comparing ES-MAML and PG-MAML \cite{ES-MAML, maml-and-universality}. Multiple potential explanations exist for this bias towards simple linear policies, including sample complexity for ES being highly dependent on the number of parameters \cite{wierstra, wierstra2011natural}, or potentially hidden layers inducing unwanted local minima in agent behaviors \cite{simplicity}. While out of the scope of this work, this interesting phenomena remains to be analyzed in finer detail.
}


\ignorethis{While the above numerical results rigorously establish the need for adaptation, in this section, we highlight the qualitative need for adaptation as well, through presentation of numerous videos for simulation.

We first note that ES-MAML is particularly biased towards compact linear policies. As shown in \href{test.com}{[Link]}, additional hidden layers in the policy bias the training towards a behavior of solving all tasks with the meta-policy, in particular with a gait that uses the Minitaur's knees rather than its legs, which clearly cannot be used in the real world case.

In addition, we highlight the various adaptations that ES-MAML provides, such as:
\begin{itemize}
\item Falling down vs Normal Walking
\item Correction of walking direction from turning to straight
\item Correcting "overfitting to the horizon length" by continuing to walk for longer horizons 
\item Linear policies producing upright walking behaviors, while Hidden layers producing Knee behaviors
\end{itemize}
}

